Beyond S-curves: Recurrent Neural Networks for Technology Forecasting

Because of the considerable heterogeneity and complexity of the technological landscape, building accurate models to forecast is a challenging endeavor. Due to their high prevalence in many complex systems, S-curves are a popular forecasting approach in previous work. However, their forecasting performance has not been directly compared to other technology forecasting approaches. Additionally, recent developments in time series forecasting that claim to improve forecasting accuracy are yet to be applied to technological development data. This work addresses both research gaps by comparing the forecasting performance of S-curves to a baseline and by developing an autencoder approach that employs recent advances in machine learning and time series forecasting. S-curves forecasts largely exhibit a mean average percentage error (MAPE) comparable to a simple ARIMA baseline. However, for a minority of emerging technologies, the MAPE increases by two magnitudes. Our autoencoder approach improves the MAPE by 13.5% on average over the second-best result. It forecasts established technologies with the same accuracy as the other approaches. However, it is especially strong at forecasting emerging technologies with a mean MAPE 18% lower than the next best result. Our results imply that a simple ARIMA model is preferable over the S-curve for technology forecasting. Practitioners looking for more accurate forecasts should opt for the presented autoencoder approach.

==> #2_IP&M_draft/snippets.tex <==
Structure (inspired by Hawkes process-based technology impact analysis):

\begin{enumerate}
    \item Why is it valid to take scientific publications as a dataset? Because we previously took patents, but scientific articles come before patents (see lag paper), so using papers we can predict even earlier
    \item Using number of articles as a proxy is valid - has been done for patents, show which other proxies have been used
    \item How was that predicted previously?
    \item theory-based approaches: mainly S-curves, lifecycle modeling/theory, fitting and then forecasting: what are S-curves, examples of research using S-curves to understand past development, and work using S-curves to forecast
    \item model-based approaches: machine learning
\end{enumerate}

- other data sources: media, web searches: not good for forecasting, but for impact analysis
- comes typically 9 years after trend is identified in scientific literature

- what are patents? explain with citation
- Patents are a direct output of R\&D activities of companies and individuals, and are thus a direct measure of technical innovation (Inventive progress measured by multi-stage patent citation analysis)
- The economical value of patents has been shown in previous work
- since there is a direct link between patents and economical value, it makes sense to predict patent values (analysis on a patent level) or the number of patents (overarching over multiple patents)
- early work counted number of patents linked to entities/concepts
- later work looked at individual patents, since patents can directly be linked to individual technologies, thus it makes sense to do that on a patent level
- patent data is readily available in the US patent data base and other databases
- patents good at identifying commercial potential of emerging areas that are tracked with other methods (Emerging technologies: quantitative identification and measurement)
- patents protects intellectual property from copying, and thus, shows direct economic interest in using a technology (INDICATORS AND THE RELATIONS BETWEEN SCIENCE AND TECHNOLOGY)

- direct link between concrete economic benefit and basic research is harder to establish
- so why look at publications?
- scientific work leads patents by 4-5 years and trends in scientific articles are predictive of trends in patents (Emerging technologies: quantitative identification and measurement)
- related work has shown a direct link between patents and scientific publications: sometimes patents are claimed by the researching institution itself, countries with highest number of publications are also countries with highest number of patents
- university research feeds invention and innovation and does not substitute it (Academic patents as an indicator of useful research? Martin Meyer)
- number of citations of us based scientific articles and us patents has increased in recent years, indicating a growing relationship between science and technology (Global and domestic utilization of industrial relevant science: patent citation analysis of science–technology interactions and knowledge flows)
- so all in all, by using scientific publications as a dataset, we are 

- directly via performance metrics: cost, power, energy consumption, number of transistors on a CPU
- In A functional approach for studying technological progress: Application to information technology the authors create a database for functional performance metrics, technologies included are structured along three dimensions: storage, transport, and transformation (cables, disks, CPUs)
- In Empirically grounded technology forecasts and the energy transition authors use forecasts costs of future energy systems
- In Quantitative empirical trends in technical performance the authors forecast 28 technological domains using performance metrics to quantify story capabilities, transportation capabilities, and transformation capabilities
- in Technological change and petroleum exploration in the Gulf of Mexico authors use drilling costs and oil and gas output to analyze the technological change in the oil and gas industry
- advantage: direct measurement of technological progress since direct metrics used, direct effects
- problem: not possible for early technologies where data does not exist, technology needs to "establish" itself first, not all technological progress is measurable directly

- indirectly via bibliographic metrics: citations (patents, scientific publications, and other publications), count
- count: number of scientific publications most important metric to gauge activity in a field Publications and patents in nanotechnology Publications and patents in nanotechnology
- citation analysis shortfalls: high citation count does not mean economic usefulness, high citation can also be for documents that best summarize a technology TRACING THE KNOWLEDGE TRANSFER FROM SCIENCE TO TECHNOLOGY AS REFLECT
- count analysis shortfalls: skew problem, where a small fraction of patents or papers get most citation, taking the count equals that out Inventive progress measured by multi-stage patent citation analysis, but some correlation between high citation and economic and technical values has been shown, as such citation analysis makes sense Inventive progress measured by multi-stage patent citation analysis
- in Estimating Technology Performance Improvement Rates by Mining Patent Data the authors establish a link between direct measures (performance improvement rates) and indirect measures (bibliometric measures like citation centrality in the patent graph)
- quick examples of papers doing citation analysis: see zotero
- citation analysis hard to do on scientific publications, since hard to map individual publications to economic value or innovations, as shown previously
- that is why we follow the count approach

- cite zhang, it is difficult to quantify and forecast that, but even though it is hard we need to do it
- cite zhang's papers

- model-based works generally assume a life cycle model that explains the technological development in the past
- theory driven
- model/theory validated by back-testing and then used to forecast
- as shown, these life cycle models mainly are employed on count data, not on individual works/patents/citations
- Practice-Based Research Competition—Forecasting New Product Life Cycle Curves: Practical Approach and Empirical Analysis: compare in-sample fit of three different life cycle models on order volumes of 170 computer parts at Dell, use the best resulting fit to produce out of sample forecasts
- advantages: interpretable model parameters, e.g. inflection point for the S-curve
- disadvantage: assume a growth model Logistic substitution model and technological forecasting, limited accuracy in early phase of a technology when forecasting is the most interesting, cannot anticipate sudden changes of the complex system they are describing Innovation on the web: the end of the S-curve?, Early identification of emerging technologies: A machine learning approach using multiple patent indicators
- Segments forecasting into short-, medium-, and longterm forecasting depending on how many parts of the curve you want to forecast. Presents modes of competition. Introduces the logistic substitution model, where new technologies slowly replace older ones. Does this analysis with cassettes, vinyl, CDs. However, multiple problems exist: hard to identify which technology will replace an older one. Find that sometimes you can find preiodicity between new technologies which tells you when a new technlogy should emerge: Logistic Substitution Model and Technological Forecasting
- Forecasting technology diffusion: a new generalisation of the logistic model: Introduce new generalisation of logistic model. Focus on forecasting in the short-term (forecast 10-20\% of the existing data points) into the future. A lot of parameters which make the formulation flexible but also hard to handle. MAPE as accuracy of fit metric. Better fit than Bhargava and Fisher-Pry.
- First, authors define technical innovation and technical growth. Then, they explain their choice of patents as their data source. They fit an S-curve to the number of patents published for web technologies. They find, that the start can be modelled well by a S-curve, however, growth did not level off and continued linearly. They modelled this by fitting PIECEWISE a sigmoid and a linear function. Innovation on the web: the end of the S-curve?
- Talk about in which fields S-curves are applied and how they are used. Talks about concept of envelope curves of multiple S-curves which in itself is an S-curves. Thus, development is driven by multiple S-curves. However, S-curves are limited in their usability: when limited data is available (only beginning of S-curve is available) uncertainties in fits are high; and thus, utility of fit is low. If alot of data is available (S-curve is advanced a lot) certainty of fit is high, but utility for forecasting is also low, because the growth already happened. Application of S-shaped curves
- Forecasting the development of the biped robot walking technique in Japan through S-curve model analysis: fit of S-curves on the number of patents in biped robot walking to find inflection points and saturation times, do forecasts on future trends for walking robots
- Security Dynamics in Computer Science Technologies: authors demonstrate the prevalence of S-curves in 20 computer science technologies by analyzing S-curve fits, but do not proceed to do forecasts

- data-driven approaches search for patterns appearing in the data
- empirically-driven
- as direct economic value of independent patents has been shown, many works exist on trying to forecast values of patents
- Forecasting emerging technologies using data augmentation and deep learning: defines technologies, classifies them into emerging and non emerging, scrapes associated papers, and uses a deep neural network to classify patents, compares to Gartner's Hype Cycle for performance
- Forecasting emerging technologies: A supervised learning approach through patent analysis: cluster patents into ET and NET clusters, compare different classifiers to classify patents into those clusters
- A novel approach to evaluating the business potential of intellectual properties: A machine learning-based predictive analysis of patent lifetime: machine learning model to predict the likelihood of patent survival until its expiry date, survival is associated with increases value of patent
- Early identification of emerging technologies: A machine learning approach using multiple patent indicators: forecast forward citations of patents to identify patents that might become become important patents/emerging technologies in the future
- Pre-launch new product demand forecasting using the Bass model: A statistical and machine learning-based approach: combines model-based and data-driven approaches: uses machine learning model to estimate model parameters using product attributes such as price, use sales data of US products
%- Deep context of citations using machine‑learning models in scholarly full‑text articles: compare several machine learning models to identify important citation among unimportant ones on scholarly articles

- less methods exist that forecast the aggregated metric of counts, can be likened to forecast of indices in finance that has enjoyed ample popularity due to immediate economic pay-offs when getting the forecast right. Here we see a research gap
- we employ modern approaches in this work in hopes of tackling the S-curve disadvantages: find patterns in data without prior assumption, which can include sudden changes if that is a pattern that occurs predictably in the data

- research gap: papers claim that ML approach is superior to the theory-based approach, no direct comparison has been done in previous work
- no ML methods have been employed on count data

The research gap we see is a direct comparison of model-based and data-driven approaches.
As shown, model-driven approaches offer the advantage of interpretable model parameters while making assumption that are not always correct.
Data-driven approaches aim at producing forecasts without making assumptions and thought to be more accurate.
The recent hype around machine learning has led to their application in almost every research domain.
However, their application does not always yield better results.
For example, Dacrema et al. show that simple baseline methods can make more accurate recommendations than sophisticated machine learning algorithms.
We see a similar trend in technological forecasting, where sophisticated machine learning models are developed to produce forecasts.
However, no direct comparison between these new approaches and the traditional model-based approaches has been made yet.
Therefore, with our work we aim at making a first step towards a critical analysis of the utility of these new methods and investigate if and by how much they improve upon existing model-based forecasting approaches.

- no work on count forecasting in technological forecasting but in other domains
- time series forecasting
- present work by DeepAR
- ML methods in time-series forecasting great results over baseline methods
- however, have not yet been applied in technological forecasting context
- we aim at applying this previously successful approach and comparing it to more traditional approaches: model-based S-curve.

Therefore, with our work aim at making a first step towards a critical analysis of the utility of these new methods and investigate if and by how much they improve upon existing model-based forecasting approaches.

- producing ARIMA forecasts
- data: run hyperparameter search on each window to find best arima configuration for each window
- that is how a practitioner would do it: take the time series up until current time, find best arima configuration using hyperparameter search, forecast
- forecast: same as in S-curves, three years

==> snippets.tex <==
Structure (inspired by Hawkes process-based technology impact analysis):

\begin{enumerate}
    \item Why is it valid to take scientific publications as a dataset? Because we previously took patents, but scientific articles come before patents (see lag paper), so using papers we can predict even earlier
    \item Using number of articles as a proxy is valid - has been done for patents, show which other proxies have been used
    \item How was that predicted previously?
    \item theory-based approaches: mainly S-curves, lifecycle modeling/theory, fitting and then forecasting: what are S-curves, examples of research using S-curves to understand past development, and work using S-curves to forecast
    \item model-based approaches: machine learning
\end{enumerate}

- other data sources: media, web searches: not good for forecasting, but for impact analysis
- comes typically 9 years after trend is identified in scientific literature

- what are patents? explain with citation
- Patents are a direct output of R\&D activities of companies and individuals, and are thus a direct measure of technical innovation (Inventive progress measured by multi-stage patent citation analysis)
- The economical value of patents has been shown in previous work
- since there is a direct link between patents and economical value, it makes sense to predict patent values (analysis on a patent level) or the number of patents (overarching over multiple patents)
- early work counted number of patents linked to entities/concepts
- later work looked at individual patents, since patents can directly be linked to individual technologies, thus it makes sense to do that on a patent level
- patent data is readily available in the US patent data base and other databases
- patents good at identifying commercial potential of emerging areas that are tracked with other methods (Emerging technologies: quantitative identification and measurement)
- patents protects intellectual property from copying, and thus, shows direct economic interest in using a technology (INDICATORS AND THE RELATIONS BETWEEN SCIENCE AND TECHNOLOGY)

- direct link between concrete economic benefit and basic research is harder to establish
- so why look at publications?
- scientific work leads patents by 4-5 years and trends in scientific articles are predictive of trends in patents (Emerging technologies: quantitative identification and measurement)
- related work has shown a direct link between patents and scientific publications: sometimes patents are claimed by the researching institution itself, countries with highest number of publications are also countries with highest number of patents
- university research feeds invention and innovation and does not substitute it (Academic patents as an indicator of useful research? Martin Meyer)
- number of citations of us based scientific articles and us patents has increased in recent years, indicating a growing relationship between science and technology (Global and domestic utilization of industrial relevant science: patent citation analysis of science–technology interactions and knowledge flows)
- so all in all, by using scientific publications as a dataset, we are 

- directly via performance metrics: cost, power, energy consumption, number of transistors on a CPU
- In A functional approach for studying technological progress: Application to information technology the authors create a database for functional performance metrics, technologies included are structured along three dimensions: storage, transport, and transformation (cables, disks, CPUs)
- In Empirically grounded technology forecasts and the energy transition authors use forecasts costs of future energy systems
- In Quantitative empirical trends in technical performance the authors forecast 28 technological domains using performance metrics to quantify story capabilities, transportation capabilities, and transformation capabilities
- in Technological change and petroleum exploration in the Gulf of Mexico authors use drilling costs and oil and gas output to analyze the technological change in the oil and gas industry
- advantage: direct measurement of technological progress since direct metrics used, direct effects
- problem: not possible for early technologies where data does not exist, technology needs to "establish" itself first, not all technological progress is measurable directly

- indirectly via bibliographic metrics: citations (patents, scientific publications, and other publications), count
- count: number of scientific publications most important metric to gauge activity in a field Publications and patents in nanotechnology Publications and patents in nanotechnology
- citation analysis shortfalls: high citation count does not mean economic usefulness, high citation can also be for documents that best summarize a technology TRACING THE KNOWLEDGE TRANSFER FROM SCIENCE TO TECHNOLOGY AS REFLECT
- count analysis shortfalls: skew problem, where a small fraction of patents or papers get most citation, taking the count equals that out Inventive progress measured by multi-stage patent citation analysis, but some correlation between high citation and economic and technical values has been shown, as such citation analysis makes sense Inventive progress measured by multi-stage patent citation analysis
- in Estimating Technology Performance Improvement Rates by Mining Patent Data the authors establish a link between direct measures (performance improvement rates) and indirect measures (bibliometric measures like citation centrality in the patent graph)
- quick examples of papers doing citation analysis: see zotero
- citation analysis hard to do on scientific publications, since hard to map individual publications to economic value or innovations, as shown previously
- that is why we follow the count approach

- cite zhang, it is difficult to quantify and forecast that, but even though it is hard we need to do it
- cite zhang's papers

- model-based works generally assume a life cycle model that explains the technological development in the past
- theory driven
- model/theory validated by back-testing and then used to forecast
- as shown, these life cycle models mainly are employed on count data, not on individual works/patents/citations
- Practice-Based Research Competition—Forecasting New Product Life Cycle Curves: Practical Approach and Empirical Analysis: compare in-sample fit of three different life cycle models on order volumes of 170 computer parts at Dell, use the best resulting fit to produce out of sample forecasts
- advantages: interpretable model parameters, e.g. inflection point for the S-curve
- disadvantage: assume a growth model Logistic substitution model and technological forecasting, limited accuracy in early phase of a technology when forecasting is the most interesting, cannot anticipate sudden changes of the complex system they are describing Innovation on the web: the end of the S-curve?, Early identification of emerging technologies: A machine learning approach using multiple patent indicators
- Segments forecasting into short-, medium-, and longterm forecasting depending on how many parts of the curve you want to forecast. Presents modes of competition. Introduces the logistic substitution model, where new technologies slowly replace older ones. Does this analysis with cassettes, vinyl, CDs. However, multiple problems exist: hard to identify which technology will replace an older one. Find that sometimes you can find preiodicity between new technologies which tells you when a new technlogy should emerge: Logistic Substitution Model and Technological Forecasting
- Forecasting technology diffusion: a new generalisation of the logistic model: Introduce new generalisation of logistic model. Focus on forecasting in the short-term (forecast 10-20\% of the existing data points) into the future. A lot of parameters which make the formulation flexible but also hard to handle. MAPE as accuracy of fit metric. Better fit than Bhargava and Fisher-Pry.
- First, authors define technical innovation and technical growth. Then, they explain their choice of patents as their data source. They fit an S-curve to the number of patents published for web technologies. They find, that the start can be modelled well by a S-curve, however, growth did not level off and continued linearly. They modelled this by fitting PIECEWISE a sigmoid and a linear function. Innovation on the web: the end of the S-curve?
- Talk about in which fields S-curves are applied and how they are used. Talks about concept of envelope curves of multiple S-curves which in itself is an S-curves. Thus, development is driven by multiple S-curves. However, S-curves are limited in their usability: when limited data is available (only beginning of S-curve is available) uncertainties in fits are high; and thus, utility of fit is low. If alot of data is available (S-curve is advanced a lot) certainty of fit is high, but utility for forecasting is also low, because the growth already happened. Application of S-shaped curves
- Forecasting the development of the biped robot walking technique in Japan through S-curve model analysis: fit of S-curves on the number of patents in biped robot walking to find inflection points and saturation times, do forecasts on future trends for walking robots
- Security Dynamics in Computer Science Technologies: authors demonstrate the prevalence of S-curves in 20 computer science technologies by analyzing S-curve fits, but do not proceed to do forecasts

- data-driven approaches search for patterns appearing in the data
- empirically-driven
- as direct economic value of independent patents has been shown, many works exist on trying to forecast values of patents
- Forecasting emerging technologies using data augmentation and deep learning: defines technologies, classifies them into emerging and non emerging, scrapes associated papers, and uses a deep neural network to classify patents, compares to Gartner's Hype Cycle for performance
- Forecasting emerging technologies: A supervised learning approach through patent analysis: cluster patents into ET and NET clusters, compare different classifiers to classify patents into those clusters
- A novel approach to evaluating the business potential of intellectual properties: A machine learning-based predictive analysis of patent lifetime: machine learning model to predict the likelihood of patent survival until its expiry date, survival is associated with increases value of patent
- Early identification of emerging technologies: A machine learning approach using multiple patent indicators: forecast forward citations of patents to identify patents that might become become important patents/emerging technologies in the future
- Pre-launch new product demand forecasting using the Bass model: A statistical and machine learning-based approach: combines model-based and data-driven approaches: uses machine learning model to estimate model parameters using product attributes such as price, use sales data of US products
%- Deep context of citations using machine‑learning models in scholarly full‑text articles: compare several machine learning models to identify important citation among unimportant ones on scholarly articles

- less methods exist that forecast the aggregated metric of counts, can be likened to forecast of indices in finance that has enjoyed ample popularity due to immediate economic pay-offs when getting the forecast right. Here we see a research gap
- we employ modern approaches in this work in hopes of tackling the S-curve disadvantages: find patterns in data without prior assumption, which can include sudden changes if that is a pattern that occurs predictably in the data

- research gap: papers claim that ML approach is superior to the theory-based approach, no direct comparison has been done in previous work
- no ML methods have been employed on count data

The research gap we see is a direct comparison of model-based and data-driven approaches.
As shown, model-driven approaches offer the advantage of interpretable model parameters while making assumption that are not always correct.
Data-driven approaches aim at producing forecasts without making assumptions and thought to be more accurate.
The recent hype around machine learning has led to their application in almost every research domain.
However, their application does not always yield better results.
For example, Dacrema et al. show that simple baseline methods can make more accurate recommendations than sophisticated machine learning algorithms.
We see a similar trend in technological forecasting, where sophisticated machine learning models are developed to produce forecasts.
However, no direct comparison between these new approaches and the traditional model-based approaches has been made yet.
Therefore, with our work we aim at making a first step towards a critical analysis of the utility of these new methods and investigate if and by how much they improve upon existing model-based forecasting approaches.

- no work on count forecasting in technological forecasting but in other domains
- time series forecasting
- present work by DeepAR
- ML methods in time-series forecasting great results over baseline methods
- however, have not yet been applied in technological forecasting context
- we aim at applying this previously successful approach and comparing it to more traditional approaches: model-based S-curve.

Therefore, with our work aim at making a first step towards a critical analysis of the utility of these new methods and investigate if and by how much they improve upon existing model-based forecasting approaches.

- producing ARIMA forecasts
- data: run hyperparameter search on each window to find best arima configuration for each window
- that is how a practitioner would do it: take the time series up until current time, find best arima configuration using hyperparameter search, forecast
- forecast: same as in S-curves, three years
